Federated Learning as Variational Inference: A Scalable Expectation Propagation Approach

The canonical formulation of federated learning treats it as a distributed optimization problem where the model parameters are optimized against a global loss function that decomposes across client loss functions. A recent alternative formulation instead treats federated learning as a distributed inference problem, where the goal is to infer a global posterior from partitioned client data (Al-Shedivat et al., 2021). This paper extends the inference view and describes a variational inference formulation of federated learning where the goal is to find a global variational posterior that well-approximates the true posterior. This naturally motivates an expectation propagation approach to federated learning (FedEP), where approximations to the global posterior are iteratively refined through probabilistic message-passing between the central server and the clients. We conduct an extensive empirical study across various algorithmic considerations and describe practical strategies for scaling up expectation propagation to the modern federated setting. We apply FedEP on standard federated learning benchmarks and find that it outperforms strong baselines in terms of both convergence speed and accuracy.

==> background.tex <==


\section{Background: Federated Learning as Variational Inference}


\subsection{Optimization --- Federated Averaging}
In (standard) data-parallel machine learning, $K$ machines split the workload and form the distributed optimization problem. In a typical workflow, (1) the central node (e.g., the parameter server) broadcasts the parameters to each of the compute nodes; (2) each of the compute nodes computes the gradient estimates on a batch of local data partition, and sends the gradients to the central node; (3) the central node aggregates the gradients, performs one step of gradient descent on the parameters; and then repeats.
Despite its popularity, a naive data-parallel algorithm suffers from high communication bandwidth and lock-step synchronous updates.

Federated Averaging (FedAvg) instead relaxes some of the constraints. It lets each server perform multiple iterations of updates before aggregating parameter updates globally. This trades off communication cost with quality, as parameters become ``stale'' after multiple iterations of updates. This would lead to incorrect solutions in certain settings~\citep{al2020federated}.


\subsection{Inference --- Posterior Averaging}
\citet{al2020federated} consider an alternative Bayesian formulation. Specifically, under the uniform prior, any global posterior distribution that exists decomposes into a product of local posteriors,
\begin{equation}
\begin{aligned}
\btheta = \argmax_{\btheta}\, p(\btheta \mid \mathcal{D}) = \argmax_{\btheta}\,  \prod_k p(\btheta \mid \mathcal{D}_k).
\label{eq:fl-as-pa}
\end{aligned}
\end{equation}
This suggests that each client can separately perform approximate posterior inference. The clients then send posterior distributions to the central server. The central server receives these local posterior distributions, multiplicatively aggregates them, and returns the mode. Intuitively, this asks each client to compute a posterior distribution of model parameters. This extra information of model parameters ``uncertainties'' helps the central server decide how to aggregate model parameters.

